OnionBots: Subverting Privacy Infrastructure for Cyber Attacks

Over the last decade botnets survived by adopting a sequence of increasingly sophisticated strategies to evade detection and take overs, and to monetize their infrastructure. At the same time, the success of privacy infrastructures such as Tor opened the door to illegal activities, including botnets, ransomware, and a marketplace for drugs and contraband. We contend that the next waves of botnets will extensively subvert privacy infrastructure and cryptographic mechanisms. In this work we propose to preemptively investigate the design and mitigation of such botnets. We first, introduce OnionBots, what we believe will be the next generation of resilient, stealthy botnets. OnionBots use privacy infrastructures for cyber attacks by completely decoupling their operation from the infected host IP address and by carrying traffic that does not leak information about its source, destination, and nature. Such bots live symbiotically within the privacy infrastructures to evade detection, measurement, scale estimation, observation, and in general all IP-based current mitigation techniques. Furthermore, we show that with an adequate self-healing network maintenance scheme, that is simple to implement, OnionBots achieve a low diameter and a low degree and are robust to partitioning under node deletions. We developed a mitigation technique, called SOAP, that neutralizes the nodes of the basic OnionBots. We also outline and discuss a set of techniques that can enable subsequent waves of Super OnionBots. In light of the potential of such botnets, we believe that the research community should proactively develop detection and mitigation methods to thwart OnionBots, potentially making adjustments to privacy infrastructure.

==> crypto.tex <==
%\subsection{Bot to Bot Communication}\label{ss:crypto}

%While many current botnets lack adequate secure communications~\cite{Rossow:2013:SPM} (e.g., sending messages in plaintext) that leaves them open to hijacking, the OnionBot's communication is completely encrypted since it uses Tor and SSL. Note that the the encryption keys are unique to each link. Table~\ref{t:botnet-crypto} summarizes a number of botnet families and their lack of adequate crypto blocks~\cite{Rossow:2013:SPM} after reverse engineering. Furthermore we introduce new cryptographic blocks that enable the OnionBot to offer new services, such as a botnet-for-rent~\cite{Hund:rambot} and a distributed computation platform for rent.

%\begin{table}
%\centering
%\scalebox{1.3}{
%\begin{tabular}{ | c | c | c | c | }\hline

%	\textbf{Botnet} & \textbf{Crypto} & \textbf{Signing} & \textbf{Replay} \\ \hline
%	Miner & none & none  &  yes	\\ \hline
%	Storm & XOR & none  &  yes	\\ \hline
%	ZeroAccess v1 & RC4 & RSA 512 & yes \\ \hline
%	Zeus & chained XOR & RSA 2048 & yes \\ \hline

%\end{tabular}
%}
%\caption{Cryptographic use in different botnets.}
%\label{t:botnet-crypto}
%\end{table}



